Dropout Attacks

Dropout is a common operator in deep learning, aiming to prevent overfitting by randomly dropping neurons during training. This paper introduces a new family of poisoning attacks against neural networks named DROPOUTATTACK. DROPOUTATTACK attacks the dropout operator by manipulating the selection of neurons to drop instead of selecting them uniformly at random. We design, implement, and evaluate four DROPOUTATTACK variants that cover a broad range of scenarios. These attacks can slow or stop training, destroy prediction accuracy of target classes, and sabotage either precision or recall of a target class. In our experiments of training a VGG-16 model on CIFAR-100, our attack can reduce the precision of the victim class by 34.6% (from 81.7% to 47.1%) without incurring any degradation in model accuracy

==> Makefile <==
SHELL := /bin/bash
WORK := $(shell basename `pwd`)
MAIN = main.tex

BASE := $(basename $(MAIN))
SRCEXT := $(patsubst $(BASE).%,%,$(MAIN))
BIBFILES := $(wildcard *.bib)
STYLINK := $(notdir $(wildcard *.sty))
STYFILES := $(sort $(STYLINK) $(wildcard *.sty))
TEXFILES := $(sort $(MAIN) $(wildcard *.tex) $(STYFILES))

LATEX = pdflatex
BIBTEX = bibtex -min-crossrefs=1000
PS2PDF = ps2pdf


# by default, not extended mode
# change this to 1 if you want extended mode by default
EXTENDED ?= 0
ifeq ($(EXTENDED),1)
EXTDEF := \def\buildextended{}
else
EXTDEF := 
endif

# by default, editing marks
# change this to 0 if you want no edit marks by default
EDITING ?= 1
ifeq ($(EDITING),1)
EDITDEF := 
else
EDITDEF := \def\noeditingmarks{}
endif

all: $(BASE).pdf

# for appendix, tmp for submission
appendix: apppdf.ltx appendix.tex
	latexmk -pdf apppdf.ltx

#.headline:
#	$(MAKE) -C headline

#.images: headline/headline.eps  $(addsuffix /*.eps,$(IMAGES)) $(addsuffix /*.tex,$(IMAGES))
#	for i in $(IMAGES); do $(MAKE) -C $$i; done
#	touch $@

#graphs/%.pdf:
#	touch scripts/$(shell basename $@ .pdf).sh

%.pdf: %.eps
	perl -ne 'exit 1 unless /\n/' $< \
		|| perl -p -i -e 's/\r/\n/g' $<
	epstopdf --outfile=$@ $<

$(BASE).pdf: %.pdf: %.$(SRCEXT) $(TEXFILES) $(BIBFILES) $(PLOT_GRAPHS)
	@echo "BASE"
	@echo $?
	$(eval LTXINPUT := "$(EXTDEF)$(EDITDEF)\input{$<}")
	latexmk -pdf $(MAIN)

%.pdf: %.tex
	latexmk -pdf $<


clean:
		rm -f eval/*.aux # eval/eval3table.tex eval/graphs/* eval/scripts/*.dat
		rm -f $(BASE).ps $(BASE).pdf
		rm -f *.dvi *.aux *.log *.bbl *.blg *.lof *.lot *.toc *.bak *.out .images $(WORK).fdb_latexmk $(WORK).fls
		for i in $(IMAGES); do $(MAKE) -C $$i clean; done

